ProTEA: Programmable Transformer Encoder Acceleration on FPGA

Transformer neural networks (TNN) have been widely utilized on a diverse range of applications, including natural language processing (NLP), machine translation, and computer vision (CV). Their widespread adoption has been primarily driven by the exceptional performance of their multi-head self-attention block used to extract key features from sequential data. The multi-head self-attention block is followed by feedforward neural networks, which play a crucial role in introducing non-linearity to assist the model in learning complex patterns. Despite the popularity of TNNs, there has been limited numbers of hardware accelerators targeting these two critical blocks. Most prior works have concentrated on sparse architectures that are not flexible for popular TNN variants. This paper introduces \textit{ProTEA}, a runtime programmable accelerator tailored for the dense computations of most of state-of-the-art transformer encoders. \textit{ProTEA} is designed to reduce latency by maximizing parallelism. We introduce an efficient tiling of large matrices that can distribute memory and computing resources across different hardware components within the FPGA. We provide run time evaluations of \textit{ProTEA} on a Xilinx Alveo U55C high-performance data center accelerator card. Experimental results demonstrate that \textit{ProTEA} can host a wide range of popular transformer networks and achieve near optimal performance with a tile size of 64 in the multi-head self-attention block and 6 in the feedforward networks block when configured with 8 parallel attention heads, 12 layers, and an embedding dimension of 768 on the U55C. Comparative results are provided showing \textit{ProTEA} is 2.5$\times$ faster than an NVIDIA Titan XP GPU. Results also show that it achieves 1.3 -- 2.8$\times$ speed up compared with current state-of-the-art custom designed FPGA accelerators.

==> analytical.tex <==
\section{Analytical Model for Latency}
The parameters that affect the resource utilization and performance of FAMOUS are the tile size or number of tiles in the attention module, the number of attention heads, the sequence length, and the embedding dimension when the bit width is fixed. An analytical model was developed to establish the relationship between these parameters and latency. This model aids in estimating both latency and the value of the parameters before synthesis.
%The number of DSPs depends on the number of parallel multiplications. They are mostly used in ${QKV}_{PU}$, ${QK}_{PU}$, ${SV}_{PU}$, and $FFN$ modules. The number of BRAMs depends on the number of arrays to store data, the BRAM modes applied to them for synthesis, and how they are partitioned.
\begin{comment}
\begin{equation}
\label{eq:dsp}
\begin{split}
    No.\ of\ DSPs &= 3\times Number\_of\_Heads\times \frac{Embedding\_Dimension}{Tiles\_in\_MHA} + Number\_of\_Heads\ \times \\ &\left(\frac{Embedding\_Dimension}{Number\_of\_Heads}+Sequence\_length\right)
           + 6\times \frac{Embedding\_Dimension}{Tiles\_in\_FFN}\ + \\ &Embedding\_Dimension
\end{split} 
\end{equation} 

\begin{equation}
\label{eq:bram}
\begin{split}
    No.\ of\ BRAMs &= \frac{10\times Sequence\_length\times Embedding\_Dimension \times Bit\_width}{BRAM\_width\times BRAM\_depth} + Sequence\_length\ \times max(0.5, \\ & \left.\frac{Sequence\_length\times Bit\_width}{BRAM\_width\times BRAM\_depth}\right) + max\left(0.5, \frac{Sequence\_length\times Embedding\_Dimension\times Bit\_width}{BRAM\_width\times BRAM\_depth}\right)
           \\ & + \frac{Number\_of\_Heads\times Sequence\_length\times Embedding\_Dimension\times Bit\_width}{BRAM\_width\times BRAM\_depth} + max(0.5,  \\ & \left.\frac{Embedding\_Dimension\times Bit\_width}{BRAM\_width\times BRAM\_depth}\right) + \frac{Sequence\_length\times Tiles\ in\ MHA\times Bit\_width}{BRAM\_width\times BRAM\_depth} + \\ & Tiles\ in\ MHA\times Number\_of\_Heads\times max\left(0.5, \frac{Sequence\_length\times Bit\_width}{BRAM\_width\times BRAM\_depth}\right) + \\ & \frac{8\times Embedding\_Dimension^2 \times Bit\_width}{Tiles\ in\ FFN\times BRAM\_width\times BRAM\_depth} + Tiles\ in\ MHA\times Number\_of\_Heads\times \\ & max\left(0.5, \frac{Embedding\_Dimension\times Bit\_width}{BRAM\_width\times BRAM\_depth}\right) + \frac{Embedding\_Dimension}{Tiles\ in\ FFN}\times max(0.5, \\ & \left.\frac{Sequence\_length\times Bit\_width}{BRAM\_width\times BRAM\_depth}\right) + 4\times Embedding\_Dimension\times max\left(0.5,  \frac{Sequence\_length\times Bit\_width}{BRAM\_width\times BRAM\_depth}\right)
\end{split} 
\end{equation} 
\end{comment}

The design is modular, and each module is implemented as a function with loops. Thus, the latency of the modules depends on the loop iteration latency, which in turn depends on the loop pipeline and unrolling pragmas. %are used for optimization. Loop pipelining was used to overlap operations from different iterations. Loop unrolling was used to execute the operations within the same iteration in parallel. For a single-loop operation in the loading units, the loop is pipelined. Unrolling was not applied because the loops have high iteration counts, and parallelization will not work because of resource limitations. Even if enough resources are available, the compiler will take a long time (more than 72 hours) to bind those resources.
For the nested loops in the modules, the second loop from the last is pipelined resulting in a complete unroll of the innermost loop. The outermost loop had no pragmas to avoid complicated pipeline depth and resource requirements. Pipelined loop latency (PLL) can be calculated by equation \ref{LL}. If it is enclosed by another loop, then the total latency (TL) will be given by equation \ref{TLL}. Here, Trip\_count (TC) is the number of iterations of a loop, and the initiation interval (II) is the latency between the initiation of two consecutive iterations. Pipeline\_Depth is the latency to finish one iteration. It depends on the sequential and parallel operations executed in one iteration. Different modules of FAMOUS can have different Pipeline\_Depth (PD). The latency is measured in clock cycles (cc). 
%\vspace{-0.2cm}
%\begin{strip}
\begin{gather}
\label{LL}
%\begin{align*}
\begin{split}
   PLL =& (TC - 1)\times II + Pipeline\_Depth  \text{\cite{perform}}
\end{split} \\
\label{TLL}
\begin{split}
   TL = PLL\times Outer\_Loop\_TC \text{\cite{perform}}
\end{split}
%\begin{split}
%   LI = & [(d_{model}-1)\times 1 + PDL]\times SL % Sequence\_length Pipeline\_Depth\_Load %Load\ Biases\ for\ %Attention
%\end{split}
%\end{align*}
\end{gather} 
%\end{strip}

%\begin{equation}
%\label{TLL}
%\begin{split}
%   TL = ILL\times Outer\_Loop\_TC \text{\cite{perform}}
%\end{split} 
%\end{equation} 
%\vspace{-0.6cm}
Equation \ref{LL} \& \ref{TLL} are generalized equations, the variables of which differ for different modules of FAMOUS as shown in the following equations.
%\vspace{-0.4cm}
%\begin{equation}
%\label{LI}
%\resizebox{.9\hsize}{\height}{$
%\begin{split}
%   LI = & [(d_{model}-1)\times 1 + PDL]\times SL % Sequence\_length Pipeline\_Depth\_Load
%\end{split}%$}
%\end{equation} 
\begin{gather} 
\label{LI}
\begin{split}
   LI = & [(d_{model}-1)\times 1 + PD\_L]\times SL % Sequence\_length Pipeline\_Depth\_Load %Load\ Biases\ for\ Attention
\end{split}\\
\label{LB}
\begin{split}
   LB = (\frac{d_{model}}{h}-1)\times 1 + PD\_L %Pipeline\_Depth\_Load
\end{split}\\
\label{LIA}
\begin{split}
LIA = & [(TS-1)\times 1 +  PD\_L]\times SL  %Load\ Inputs\ %for\ Attention Sequence\_length \frac{d_{model}}%{(\frac{d_{model}}{TS})}
\end{split}\\
\label{LWA}
\begin{split}
LWA = [(\frac{d_{model}}{h}-1)\times 1 + PD\_L]\times SL
\end{split}\\
\label{MHA}
\begin{split}
   SA = [(\frac{d_{model}}{h}-1)\times 1 + PD\_MHA]\times SL % Sequence\_length Pipeline\_Depth\_MHA
\end{split}\\
\label{BA}
\begin{split}
      BA = [(\frac{d_{model}}{h}-1)\times 1 + PD\_BA]\times SL %Sequence\_length Pipeline\_Depth\_Bias\_Add Bias\_Addition
\end{split}\\
\label{s}
\begin{split}
   S = [(SL-1)\times 1 + PD\_S]\times SL % Sequence\_length\\ Pipeline\_Depth\_Score
\end{split}\\
%\end{gather}
%\begin{gather}
\label{sv}
\begin{split}
   SV = [(\frac{d_{model}}{h}-1)\times 1 + PD\_SV] \times SL %Pipeline\_Depth\_SV]\times Sequence\_length
\end{split}
\end{gather}

\begin{comment}
\begin{gather} 
%\label{LIA}
%\begin{split}
%LIA = & [(TS-1)\times 1 +  PD\_L]\times SL  %Load\ Inputs\ %for\ Attention Sequence\_length \frac{d_{model}}%{(\frac{d_{model}}{TS})}
%\end{split}\\
\label{LWA}
\begin{split}
LWA = [(\frac{d_{model}}{h}-1)\times 1 + PD\_L]\times SL
\end{split}\\
\label{MHA}
\begin{split}
   SA = [(\frac{d_{model}}{h}-1)\times 1 + PD\_MHA]\times SL % Sequence\_length Pipeline\_Depth\_MHA
\end{split}\\
\label{BA}
\begin{split}
      BA = [(\frac{d_{model}}{h}-1)\times 1 + PD\_BA]\times SL %Sequence\_length Pipeline\_Depth\_Bias\_Add Bias\_Addition
\end{split}\\
\begin{split}
   S = [(SL-1)\times 1 + PD\_S]\times SL % Sequence\_length\\ Pipeline\_Depth\_Score
\end{split}\\
\begin{split}
   SV = [(\frac{d_{model}}{h}-1)\times 1 + PD\_SV] \times SL %Pipeline\_Depth\_SV]\times Sequence\_length
\end{split}
\end{gather}
\end{comment}

where, PD\_L includes the time required to establish communication with HBM using AXI master interface (7 cc), read address location (1 cc), load (1 cc), and store (1 cc) data from and to that address, and convert floating point data to fixed point (3 cc) for tasks such as loading all inputs (LI) and all biases (LB), as well as loading inputs (LIA) and weights (LWA) for each attention head. PD\_MHA equals ($\frac{d_{model}}{TS}$) plus the time required to load (1 cc), multiply (2 cc), add (1 cc), and store (1 cc) for computing self-attention (SA) in $QKV_{PM}$ module. PD\_BA includes latency associated with loading, adding, and storing operations in bias addition (BA) tasks. PD\_S equals ($\frac{d_{model}}{h}$), the time required to compute the score (S) in $QK_{PM}$ module. PD\_SV equals SL in the computation of SV within the $SV_{PM}$ module. Experimental results showed that 

Equation \ref{total_cc} represents the total latency ($LAT_{total}$) in clock cycles (cc), which was calculated by summing equations \ref{LI} through \ref{sv}. Equation \ref{total_ms} converts clock cycles into milliseconds (ms).

\vspace{-0.3cm}
\begin{gather} 
\label{total_cc}
\begin{split}
   LAT_{total}(cc) = & LI+LB+LIA+LWA+ \\& SA+BA+S+SV
\end{split}\\
\label{total_ms}
\begin{split}
   LAT_{total}(ms) = & \frac{LAT_{total}(cc) \times 10^{3}} {Frequency \ (Hz)}
\end{split}
\end{gather}
For instance, the analytical model predicts a latency of 0.98 ms at 400 MHz for the configuration of test 1 in Table \ref{results-overall}, closely matching the experimental result of 0.94 ms. Likewise, for test 6, the analytical model estimates a latency of 1.9 ms, which is very close to the 2 ms observed experimentally. Other data from the same table will also comply with the analytical model.
\begin{comment}
\begin{equation*} 
\label{soft}
\begin{split}
   softmax &= [(Sequence\_length-1)\times 1 + Load + Store]\times Sequence\_length + [(Sequence\_length-1)\times 1  \\ & +Load + Store + add + exponentiation]\times Sequence\_length + [(Sequence\_length-1)\times 2 \\ & 
     + Load + Store + divide]\times Sequence\_length
\end{split} 
\end{equation*} 
\end{comment}



==> model.tex <==
\section{Model Selection}\label{model}
The LSTM model is chosen for a high-rate dynamic system to predict the real-time response within microsecond latency. The experimental data known as DROPBEAR was generated by Joyce et al.\cite{testbed}. The test setup and data are described in \cite{high-rate4, atiyeh}. % and shown in Fig.~\ref{DROP}.
Various LSTM models were trained on Python with Tensorflow and Keras to find a suitable model that meets the RTOS requirement of 500~$\mu$s in a real-time device consisting of a cRIO-9035 with a 1.33 GHz dual-core Intel Atom (E3825) manufactured by NI. %Training used an early stopping scheme which halted training after the model was sufficiently converged. It used an Adam optimizer with a learning rate 0.0005. In this paper, we showed that FPGA implementation can outperform the RTOS for the same model. We also showed what effects different FPGA implementation methods have on performance and cost.
\begin{comment}
\begin{figure}[h!]
\centering
%\includegraphics[width=1\linewidth]{figures/arch-n.png}
\includegraphics[height=3.5cm, width=1.0\linewidth]{figures/DROPBEAR_Setup.png}
\caption{\label{DROP}DROPBEAR Test Setup with Displacement Input and Measured Acceleration\cite{data}.}
\end{figure}
\end{comment}
% JDB: modifed this paragraph
The number of units per LSTM layer was varied from 8 to 40 units, each layer having the same number of units for simplicity. The number of layers was swept from 1 to 3. Fig.~\ref{SNR} shows a large variance in the measurement of signal-to-noise ratio (SNR) as we vary units per layer, though the SNR improves with increased number of layers. The 3-layer configuration with 15 units/layer is chosen in this paper for FPGA implementation as it has the highest SNR.
%, and the size is small enough for rapid training and real-time inference.
The model has 16 input features sourced from the input signal uniformly sampled across the previous timestep and produces an output state prediction every 500~$\mu$s on RTOS.


==> rebuttal.tex <==
\section{Rebuttal Response}
\begin{center}
\textbf{----------------------- REVIEW 1 ---------------------}\end{center}
\begin{center}
\textbf{Questions for Authors’ Response}\end{center}
Q1: Please discuss the implications of only running the attention layer on the FPGA - required data movements, future directions, etc. What would happen if you ran the complete neural architecture on the FPGA?\\
\textbf{Ans.:} The feedforward network following the attention layer will use the same tiling technique but with a different tile size to fit a complete transformer model on the FPGA. There may be a need to reduce the number of parallel attention heads. As a result, the latency would increase. We are currently developing a full transformer encoder for a future project using this same architectural concept. \\
Q2: Please describe the key intuition behind your architectural concept.\\
\textbf{Ans.:} The architecture is flexible enough to support most state-of-the-art transformers without requiring a complete design cycle. For this paper, the architecture supports only the attention module, but it will be expanded to support the full encoder and eventually both the encoder and decoder of the transformer. It is modular, allowing optimization of each module separately during the design phase by adjusting a few parameters within the HLS code. The tile size determines the utilization of BRAMs and DSPs.\\
Q3: please discuss prediction quality implications of post-training quantization\\
\textbf{Ans.:} Quantization for various applications might lead to accuracy loss, although it wasn't the primary focus of this work. If a larger bit width is necessary, the design can be easily adjusted by modifying certain parameters in HLS during design time, which will affect resource utilization and latency.
\hfill \\
\hfill \\
\begin{center}
\textbf{----------------------- REVIEW 2 ---------------------}\end{center}
\begin{center}
\textbf{Questions for Authors’ Response}\end{center}
1. How are the parameters dynamically adjusted during runtime and what transformer model was used for evaluation?\\
\textbf{Ans.:} The parameters are modified by software running on a Microblaze softcore processor. The Bidirectional Encoder Representation of Transformer (BERT) model was utilized for evaluation. BERT comes in different variants with varying parameters. Table I demonstrates results for different variants executed using the same accelerator.\\
2. What are the major differences of the proposed accelerator as opposed to the existing work?\\
\textbf{Ans.:} The main distinctions lie in the tiling technique, dense matrix computations, and flexibility. Since existing literature does not disclose their full design strategies and architecture, it's challenging to pinpoint architectural modifications from them, making our proposed accelerator unique.

\hfill \\
\hfill \\
\hfill \\
\hfill \\
\hfill \\
\hfill \\

\begin{center}
\textbf{----------------------- REVIEW 3 ---------------------}\end{center}
\begin{center}
\textbf{Questions for Authors’ Response}\end{center}
Firstly, the reasons for the superior performance of the proposed design compared to state-of-the-art (SOTA) works are unclear. Detailed analysis explaining the choice of design and its performance benefits should be included. Honestly, techniques such as loop unrolling, tiling, and maximizing the use of BRAMs and DSPs are commonly employed in FPGA accelerator designs. A parameterized design is also not novel. If you believe your design offers a significant contribution to the literature, please clearly demonstrate this in the manuscript. For instance, the tiling strategy remains unclear to me. Is the input tiled? If so, along which axis is it tiled, and why was that strategy chosen? Unless these questions are addressed, I believe the proposed design offers only a weak contribution.
In Section VI, the author mentions that the runtime programmable feature is advantageous because it can "run multiple applications with minimal degradation of throughput." However, the benefits of this feature are not clear to me. Running a transformer on an FPGA with low-batch data may be preferable to running it on a GPU or CPU. Yet, I see no practical scenarios where one would need to run multiple applications on an FPGA. If we need to run multiple applications involving transformers, using a GPU might be better due to its massive parallelism and the programmability of CUDA cores. In what scenarios would running multiple applications be beneficial?\\
\textbf{Ans.:} Section IV explicitly mentions that the weights for generating the query, key, and value matrices are declared as separate arrays of size (tile\_size*embedding\_dimension* number\_of\_head) in HLS. These weights are stored as a 1D array, so tiling was applied to one axis. We experimented with various tile sizes to determine an optimized value for our architecture. Additionally, the more tiling is applied, the higher the latency because each tile is computed sequentially. Therefore, our approach was to apply tiling as little as possible to maximize resource consumption and minimize latency. This level of tiling was sufficient for the attention layer in state-of-the-art models like BERT, but larger models or the full transformer may require more tiling.

When we say "Run multiple applications with minimal degradation of throughput,"  we mean that our accelerator can handle many applications with different variants of transformer models by adjusting just a few parameters dynamically at runtime. It processes one application at a time, not multiple applications simultaneously, but it's flexible enough to be configured for different applications during runtime. This flexibility reduces the time required for coding and synthesizing different designs for different models. While it's a generalized design for multiple applications, it may not perform as optimally as a custom design, but the performance degradation is minimal even with this level of generality.

\hfill \\
\hfill \\

\begin{center}
\textbf{----------------------- REVIEW 4 ---------------------}\end{center}
\begin{center}
\textbf{Questions for Authors’ Response}\end{center}
Q1.How exactly do you quantize your models and is there really no loss of accuracy due to this?\\
\textbf{Ans.:} At this stage, accuracy loss is not assessed. The experiments demonstrate the behavior of the accelerator for fixed-point precision of either 8-bit or 16-bit, as other works we compared against also concentrated on these two-bit widths. Inputs, weights, and biases are converted into fixed-point numbers with a 4-bit integer and a 4-bit fractional part using the HLS library.\\
Q2. "The works in [24], [33], and [39] reported latency for single-head attention calculation, which we adjusted for 8 attention heads." - How is this done?\\
\textbf{Ans.:} The number of operations (GOP) reported for the transformer base model in reference [39] is equivalent to the operations of a single self-attention head. It compared latency with reference [24], which may have reported latency for single-head computations based on the given resource usage and algorithm. Reference [33] also compared its results with reference [24], so it was assumed that it also measured latency and resources for single-head computation. Since our results were for 8 self-attention heads, we multiplied the results of other works by 8 for a fair comparison.


==> reviews.tex <==
\onecolumn
\section{Reviews}\label{reviews}
\begin{center}
\textbf{----------------------- REVIEW 1 ---------------------}\end{center}
SUBMISSION: 138 
TITLE: A Flexible Accelerator for the Attention Mechanism of Transformer on FPGA 
AUTHORS: Ehsan Kabir, Md Arafat Kabir, Austin R.J. Downey, Jason D. Bakos, David Andrews and Miaoqing Huang.\\
Key strengths ----------- 
Attention is at the heart of deep learning \\
Key weaknesses ----------Attention layer only, not a full DNN 
- Unclear architecture proposal 
- Incomplete comparison to related work\\
Overall evaluation ----------- 
SCORE: -2 (reject) 
----- TEXT: 
The authors propose to accelerate attention layers, as found in many neural architectures these days, by exploiting the massive parallelism of FPGAs. This is combination with tiling and post-training quantization is used for an HLS-based implementation on an FPGA. The configuration of an attention layer in terms of attention heads, embedding dimension, and sequence length remains configurable. The authors claim performance faster than Cascade-Lake CPUs and Volta-class GPUs for an implementation on a XILINX U55C (UltraScale+). 
 
It is true that attention is at the heart of deep learning, and that the underlying tensor operations makes up a large fraction of the overall time. However, if it was that simple then one would go for a large array processor to implement the underlying linear algebra operations. Instead, it is important to execute a full neural network on a device, and this is where the trade-offs come into play. To my understanding, this aspect is ignored in the present submission. 
 
Furthermore, it remains unclear what the intuition behind your proposal is. Please elaborate in much more detail, and compare also in detail against related work. The combination of massive parallelization + quantization + FPGA is not convincing, respectively has been various times before (as you state [24,33-36]). 
 
Finally, in the evolution the comparison to related work is appreciated, but it seems to me that this is based on a mix of attention configuration, technology, and full/partial execution of attention-based DNNs. In this regard, Table II compares different configurations of the attention layer, I am not sure what to take away from this table as various things are being mixed in here. 
 
Minor: 
- You claim that induced sparsity can lead to accuracy degradation - which is true. However, the same applies to post-training quantization, as it used in your work. 
- I assume GOPS refers to GOP/second 
- Regarding the flexibility supporting different attention configurations: what would be the benefit of this? I understand such neural architectures to have a lifetime long enough to easily re-implement a new configuration, in particular as this is reconfigurable hardware. I would rather expect that you try to tailor an implementation as much as possible for a given workload.
\begin{center}
----------- Questions for authors’ response ----------
\end{center}
Q1: please discuss the implications of only running the attention layer on the FPGA - required data movements, future directions, etc. What would happen if you'd run the complete neural architecture on the FPGA? \\
Q2: please describe the key intuition behind your architectural concept.\\
Q3: please discuss prediction quality implications of post-training quantization 

\hfill \\
\hfill \\

\begin{center}
\textbf{----------------------- REVIEW 2 ---------------------}    
\end{center}
SUBMISSION: 138 
TITLE: A Flexible Accelerator for the Attention Mechanism of Transformer on FPGA 
AUTHORS: Ehsan Kabir, Md Arafat Kabir, Austin R.J. Downey, Jason D. Bakos, David Andrews and Miaoqing Huang.\\
Key strengths ----------- 
1. The attention mechanism of the transformer model accounts for a significant portion of the runtime. This paper proposes a flexible FPGA-based accelerator design to accelerate the transformer model's attention mechanism. 
2. The proposed solution has achieved fair results. 
3. Overall, the paper is well organized.\\ 
Key weaknesses ----------- 
1. Writing can be improved. 
2. Requires more details on the flexibility of the accelerator.  
3. Paper presents limited novelty, and some terms are not properly defined.\\ 
Overall evaluation ----------- 
SCORE: 1 (weak accept) 
----- TEXT: 
This paper has a few problems that need to be addressed. 
 
The writing quality is average. The paper contains minor grammatical errors and several other issues that affect the paper's readability. Some terms have been used before properly defining them. For example, in Section II, Qi, Ki, Vi, and Xi are used without defining what i stands for. The authors have also used dimension sizes like tile\_size, sequence\_length, etc. which are not defined properly. Abbreviations such as DMA are left undefined, and others, like LUT, are defined after initial use. A sentence in the conclusion, “The architecture is flexible to support different topologies of the transformer at runtime without going through synthesis steps”, is redundant.  
 
Inconsistencies are present throughout the paper. For instance, in Section II, the authors mention that there are two linear transformations in the position-wise feed-forward network. However, they have only described the first linear transformation. There is no mention of a second linear transformation. Moreover, they have introduced the query, key, and value as matrices and later described them as vectors. In the Introduction, the authors have stated that HLS “lacks the ability to effectively manage certain FPGA resources required for optimal functionality, such as DSP resources on a FPGA”. This claim is contradictory, given that in Section IV, they present an HLS design that generates an optimized architecture utilizing most of the BRAMs and DSPs. The authors state that there are three separate modules in the accelerator. However, they also describe other separate modules that are used for weight and bias loading and adding the biases. Hence, it is not clear whether th 
ere are 6 modules altogether. 
 
There are some missing details and discussions in Sections III, V and VI of the paper. A major claim of the paper is the flexibility of the accelerator. However, to support this claim, more discussions are required on how parameters can be dynamically adjusted during runtime. In section III, although the authors have identified a few existing works in the domain, a comparison of how they differ from the proposed solution is lacking. In Section V, the authors have claimed that BERT is the largest language model, which I believe is incorrect. They mention that the sequence length of the accelerator is configured to a maximum value of 64 according to the BERT model. Yet, the BERT model has a maximum sequence length of 512. It is unclear if these maximum values are for the tiled computations. In Section VI, although the authors claim the maximum sequence length configured is 64, they have presented results with a sequence length of 128.  Moreover, in Section VI, it is unclear which transformer model was used to evaluate the accelerator performance, as nothing has been stated about it. Also, the authors have not properly defined how the metrics, latency and throughput, were computed. 
\begin{center}
----------- Questions for authors’ response -----------
\end{center}
1. How are the parameters dynamically adjusted during runtime and what transformer model was used for evaluation? \\
2. What are the major differences of the proposed accelerator as opposed to the existing work? 
\hfill \\
\hfill \\
\begin{center}
\textbf{----------------------- REVIEW 3 ---------------------}\end{center}
SUBMISSION: 138 
TITLE: A Flexible Accelerator for the Attention Mechanism of Transformer on FPGA 
AUTHORS: Ehsan Kabir, Md Arafat Kabir, Austin R.J. Downey, Jason D. Bakos, David Andrews and Miaoqing Huang.\\
Key strengths ----------- 
This paper presents two main strengths in its approach to enhancing the attention mechanism of transformer neural networks on FPGA platforms. 
The proposed accelerator efficiently leverages FPGA resources, such as BRAMs and DSPs to improve parallel processing capabilities. By using high-level synthesis tools, the design optimizes the arrangement and usage of on-chip memory and processing elements, which enables it to handle large matrix computations effectively and with reduced latency. 
Also, the proposed accelerator architecture supports runtime programmability of key parameters, including the number of attention heads, tile size, and embedding dimensions. This feature allows it to adapt dynamically to different transformer topologies without the need for re-synthesis, making it highly versatile for various applications. \\
Key weaknesses ----------- 
The proposed tiling strategy for MHA (Multi-Head Attention) shows limited novelty. To enhance its originality, tiling could be applied across multiple dimensions, complemented by a thorough design space exploration. Additionally, the choice of a tiling size of 64 needs stronger justification, considering potential for optimization. 
The impact of proposed design’s runtime programmability on performance also merits examination, especially in comparison to modern devices with advanced reconfigurability features like those from Xilinx (e.g. dynamic partial reconfiguration).\\
Overall evaluation ----------
SCORE: -2 (reject) 
----- TEXT: 
This paper introduces parallelism in MHA computation and achieves better latency compared to both GPU and CPU. Tiling of input data and weight fused with quantization is helping efficient use of BRAMs available on FPGA. On top of these, the proposed design uses parameterized HLS code to ensure the design time modification functionality which is crucial for deploying transformers efficiently across different deployment scenarios and requirements. However, there are few potential weaknesses in the manuscript. 
The employment of a tiling strategy to fit input data into FPGA buffers is a well-established technique. I believe there is limited novelty in their approach. To enhance the novelty, it would be beneficial if tiling were applied and tested along different axes. Additionally, a thorough analysis of design space exploration should be included to substantiate the effectiveness and originality of their tiling strategy. Focusing solely on the embedding dimension for tiling appears somewhat naive. Exploring tiling strategies across various dimensions, such as weights or specific input dimensions, would significantly enrich the contribution to the literature. For example, [1] already successfully implemented an inference accelerator with tiling in MHA. With a unified matrix processing engine, they optimized the tiling strategy by testing at least three dimensions (M, K, N) in the matrix multiplication. 
Furthermore, the legitimacy of selecting the best parallelism design parameter, particularly the tiling size of 64 — whether for minimizing latency or maximizing throughput — is not well-supported. The rationale behind this choice seems to be based merely on the over-utilization of LUTs or compilation time constraints. There is potential to further optimize design parameters to enhance performance. 
While runtime programmability is advantageous for design reuse, it is important to consider its impact on performance. Does this functionality introduce any overhead? Although FPGAs are known for their reconfigurability, this feature does come at a cost. Modern FPGA devices, such as those in Xilinx's data center cards, even allow for on-the-fly configuration swaps. How does the proposed adaptability compare to these advanced reconfigurability features in terms of energy efficiency and performance (e.g. latency)? 
[1] Zeng, Shulin, et al. "FlightLLM: Efficient Large Language Model Inference with a Complete Mapping Flow on FPGAs." Proceedings of the 2024 ACM/SIGDA International Symposium on Field Programmable Gate Arrays. 2024. 
\begin{center}
----------- Questions for authors’ response ----------- \end{center}
Firstly, the reasons for the superior performance of the proposed design compared to state-of-the-art (SOTA) works are unclear. Detailed analysis explaining the choice of design and its performance benefits should be included. Honestly, techniques such as loop unrolling, tiling, and maximizing the use of BRAMs and DSPs are commonly employed in FPGA accelerator designs. A parameterized design is also not novel. If you believe your design offers a significant contribution to the literature, please clearly demonstrate this in the manuscript. For instance, the tiling strategy remains unclear to me. Is the input tiled? If so, along which axis is it tiled, and why was that strategy chosen? Unless these questions are addressed, I believe the proposed design offers only a weak contribution. 
In Section VI, the author mentions that the runtime programmable feature is advantageous because it can "run multiple applications with minimal degradation of throughput." However, the benefits of this feature are not clear to me. Running a transformer on an FPGA with low-batch data may be preferable to running it on a GPU or CPU. Yet, I see no practical scenarios where one would need to run multiple applications on an FPGA. If we need to run multiple applications involving transformers, using a GPU might be better due to its massive parallelism and the programmability of CUDA cores. In what scenarios would running multiple applications be beneficial? 
 
\hfill \\
\hfill \\
\begin{center}
\textbf{----------------------- REVIEW 4 ---------------------}\end{center}
SUBMISSION: 138 
TITLE: A Flexible Accelerator for the Attention Mechanism of Transformer on FPGA 
AUTHORS: Ehsan Kabir, Md Arafat Kabir, Austin R.J. Downey, Jason D. Bakos, David Andrews and Miaoqing Huang.\\
Key strengths ----------- 
Acceleration of an important building block of modern neural networks: The attention mechanism 
- Evaluation/Comparison against CPU, GPU, ASIC and other FPGA accelerators from literature 
- Adequate explanation of the Transformer architecture in the background section\\
Key weaknesses ----------- 
- Only core attention operation implemented, not a complete Transformer block or entire Transformer model 
- HLS implementation not described in detail and lacks innovation 
- Unclear fairness of comparison against other architectures as area and energy efficiency are not reported 
- Presentation contains some questionable statements and contradictions\\ 
Overall evaluation ----------- 
SCORE: -1 (weak reject) 
----- TEXT: 
The paper presents an HLS accelerator design for the inference of the attention mechanism found in Transformer models. While the topic is highly relevant and the results seem competitive, the HLS design at the core of this work is described on an abstract level and does not seem to contain innovations on the algorithmic or architectural level. The quantization is especially underspecified, as it is unclear which parts of the model (inputs, weights, activations, softmax computation) is quantized and how the quantization is performed. No loss of accuracy is reported for 8-bit quantization, but this is not believable without data to back it up. For the system implementation (section V.), the interplay between host, HBM, controller, and MicroBlaze is not clear (e.g., is the MicroBlaze used solely for latency measurement?). 
 
The evaluation compares against ASIC, GPU, CPU, as well as alternative FPGA accelerators, which is admirable. Unfortunately it is not clear how fair this comparison truly is, as the quantization between implementations varies and neither accuracy, nor area or energy efficiency are reported. It is also unclear if the demonstrated performance would scale to a real Transformer, which might contain other bottlenecks besides the attention operation itself. 
 
As far as the presentation is concerned, the paper is mostly easy to read and contains suitable figures and tables. However, the "Introduction" section fails to put the work into a meaningful context of accelerating the attention mechanism on an FPGA. While a lot of relevant information is given (referenced), for example starting by enumerating various variants of transformer model or mentioning the different types of accelerators (GPUs, CPUs, ASICs, FPGAs), it is difficult to find a clear line of thought. Some facts feel out of context or are phrased weirdly, like the "significant portion of the runtime" referenced form the cited "ELSA" paper [13]: The specific numbers given (38\%, 64\%, 4x) are hard to interpret without specifying what the sequence lengths are, what is actually measured/compared. Also, statements like "general-purpose platforms like GPUs and CPUs lack the capability to speed up such computationally demanding attention mechanisms" are at least partially misleading/out of context, as GPUs are still the dominating accelerator with full support for the attention mechanism. The memory required to store the BERT matrices cannot be stated as a simple fact as it is, as this relies on assumptions regarding model hyper-parameters and the numerical representation chosen to store these weights (probably assuming floating-point here, but there is a lot of work regarding low bit-width quantization which is seemingly neglected here which could significantly bring down this number). Also the relation of this matrix size to BRAM and partitioning/tiling could benefit from some explanations, as it relies on assumptions on how matrix computations are scheduled on an FPGA. The paragraph on HLS vs. HDL is well-intentioned, but fails to explain the authors choice for implementing their accelerator via HLS. 
 
Other minor comments: 
- Fig. 3 not referenced in text 
- It is not explained why Fig. 4 shows two separate UART blocks 
- Table II: 71 GOPS for the Nvidia V100 and 280 for the Intel E5 does not seem right , maybe you mixed up the columns? Please check. 
- Section V "Overall System": "according to the largest SOTA transformers attention layer known as BERT" - BERT is by far not the largest SOTA transformer model, the largest models are probably the recent iterations from the GPT family. 
- No future work mentioned 
\begin{center}
----------- Questions for authors’ response ----------- \end{center}
- How exactly do you quantize your models and is there really no loss of accuracy due to this? 
- "The works in [24], [33], and [39] reported latency for single-head attention calculation, which we adjusted for 8 attention heads." - How is this done? 
 

==> system.tex <==
%\vspace{-0.5cm}
\section{Overall System}\label{system}

Fig.~\ref{System} shows the complete system design for running the multi-head attention layer on different FPGA platforms such as U200 (UltraScale+XCU200-FSGD2104-2-E) and U55C (UltraScale+XCU55C-FSVH2892-2L-E) for our experiments. Each design parameter can be programmed during runtime up to a maximum value by MicroBlaze ($\mu$B) softcore processor. 
\begin{figure}[h]
\centering
%\includegraphics[width=1\linewidth]{figures/arch-n.png}
\includegraphics[height=4cm, width=0.8\linewidth]{figures/Complete_System_mha3.png}
\caption{\label{System}Complete System Design}
\end{figure}

\begin{figure*}[t]
\centering
%\includegraphics[width=1\linewidth]{figures/arch-n.png}
\includegraphics[height=5cm, width=0.8\linewidth]{figures/isa5.pdf} % 6cm 0.7cm
\caption{\label{isa} Process for Incorporating Programmability.}
\end{figure*}

The overall system was designed on Vivado 2022.1.2 design suite. It contains a custom IP block for the MHA accelerator, which is exported from HLS. The inputs and weights are fetched from off-chip high-bandwidth memory (HBM) using AXI4 master interfaces \cite{axiMaster} when the load instruction from the accelerator controller is received according to demand. The accelerator receives control signals from the processor through an AXI-lite slave interface. $\mu$B can access the HBMs which is connected to the MHA accelerator. It is used to transfer data to the BRAMs from HBMs. It also sends control signals to the accelerator. The boards are connected to a host PC with USB-JTAG interface and PCIe 3.0$\times$4 interface. This host can communicate with other IPs except $\mu$B using the DMA/Bridge Subsystem for PCI Express IP \cite{DMA} in the system, but PCI communication was not needed in this work. $\mu$B uses AXI-TIMER\cite{axitimer} to measure the latency, which includes the time between the start and stop signal from the custom IP module. The host connected to JTAG cable\cite{jtag} displays the results on the terminal using the UARTlite interface\cite{axiuart}. 






